Reading Strategies for Graph Visualizations that Wrap Around in Torus Topology

We investigate reading strategies for node-link diagrams that wrap around the boundaries in a flattened torus topology by examining eye tracking data recorded in a previous controlled study. Prior work showed that torus drawing affords greater flexibility in clutter reduction than traditional node-link representations, but impedes link-and-path exploration tasks, while repeating tiles around boundaries aids comprehension. However, it remains unclear what strategies users apply in different wrapping settings. This is important for design implications for future work on more effective wrapped visualizations for network applications, and cyclic data that could benefit from wrapping. We perform visual-exploratory data analysis of gaze data, and conduct statistical tests derived from the patterns identified. Results show distinguishable gaze behaviors, with more visual glances and transitions between areas of interest in the non-replicated layout. Full-context has more successful visual searches than partial-context, but the gaze allocation indicates that the layout could be more space-efficient.

==> sections/discussion.tex <==
\section{discussion}
% We investigate the research questions. 
% \tnocontext{} layout adopts strategy of more frequent glance saccades after immediately fixated areas, and has significantly more transitions between two or more density kernels (clusters of fixation points) than all the other layout conditions.
% We suggest to automatically center content of interest to avoid the visual cut.
% In \tpartialcontext{}, frequent visual searches over redundant areas are identified. 
% In \tfullcontext{} the visual search concentrates on one or two complete shortest paths leading to more effective performance in time, but the large screen space is quite inefficient based on scanpaths. 

% Our approach is exploratory data analysis. We do not have pre-identified gaze metrics. Rather, we begin to establish the required metrics for quantifying specific gaze patterns found during the exploratory analysis (see~\autoref{sec:methods}).

% This suggests that if we could bring content of interest to centre and avoid link wrapping, the improved aesthetics (visual clutter) may lead to improvement of graph reading.

% Limited sample size in statistical sense.
% Build hypothesis before running the ET study. 
% Our results show there is more frequent glance saccades involved in AOI transitions. 
% We may hypothesise that in none replicated layout it has longer average saccade length than fully and partially replicated layouts due to more visual searchese across AOIs.
% However, our evaluation shows that this is not reflected from the current eye tracking analysis results.
% By looking at the resolution of the graph layout shown in each stimuli, the size of the graph allocated for none replicated layout is the same as the central tile in fully replicated and partially replicated torus layouts. 
% The difference in the layouts, which means none replicated layout consumes smaller screen space than the other two conditions.
% This makes the comparison of average saccade length inconclusive in this study. 
% Future study could further evaluate this and 

